Combinatorial Abstractions of Dynamical Systems

Formal verification has been successfully developed in computer science for verifying combinatorial classes of models and specifications. In like manner, formal verification methods have been developed for dynamical systems. However, the verification of system properties, such as safety, is based on reachability calculations, which are the sources of insurmountable complexity. This talk addresses indirect verification methods, which are based on abstracting the dynamical systems by models of reduced complexity and preserving central properties of the original systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{Bortolussi, Bujorianu, Pola (Eds.): HAS 2013\\
EPTCS 124, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.124.2}{10.4204/EPTCS.124.2}}

